Calculation of supercritical Dirac resonances in heavy-ion collisions

This resonance is similar in character to other resonances in atomic physics. It is parameterized by its energy and its lifetime. A numerical discretization technique, the mapped Fourier grid method (MFG) is extended to the Dirac equation and is used to solve for the resonance parameters of a quasimolecular supercritical 1S$\sigma$ state which arises, e.g., in a uranium-uranium collision. Direct methods using only the MFG method are shown to give reasonable estimates for the resonance parameters. Analytic continuation methods such as complex scaling (CS) of the coordinate or adding a complex absorbing potential (CAP) are then applied. They allow for more accurate determinations of the supercritical resonance parameters. The (extrapolated) augmented analytic continuation methods are used to investigate the effects of higher-order couplings, beyond the monopole approximation. For the nearly charge symmetric system of U$^{92+}$-Cf$^{98+}$, it is shown that the S-D quadrupole coupling is the next dominant interaction after the monopole interaction. Collisions near the Coulomb barrier, in which supercritical resonance states occur, are also calculated using the MFG. Results are presented for the collision of U$^{92+}$-U$^{92+}$ for a zero-impact-parameter Coulomb trajectory at a center-of-mass energy of 740MeV. The enhancement effects to the positron spectrum due to nuclear sticking at closest approach is examined. Results are given for sticking times of 2,5,10$\times10^{-21}$s. Nuclear sticking is shown to offer the possibility of demonstrating experimentally the existence of supercritical resonance states.

==> Acknow.tex <==
First and foremost, I would like to thank my incredible wife Bonnie. Your love and support made all this possible. Your support never wavered, and you always had words of encouragement and a loving smile. 

To Marko Horbatsch, thank you for your guidance, advice and most of all your patience. Your wisdom and careful methodology has taught me to balance the fine details of the research with the broader context to which the research is a part of. I thank you for your patience in guiding me from a rather brash and unfocus novice to a more seasoned amateur. I sincerely appreciate the trust you placed in me by remaining at arms length allowing me to pursue areas I found of interest, all the while guiding me along. I would also like to thank you for your honest criticisms and willingness to spend the time to properly explain things to me. 

To Jurij Darewych and Roman Koniuk, thanks for all the help, guidance and your patience. The invaluable experiences of the research reviews made any other academic evaluation seem easy. Also, thank you both for all the letters of recommendation allowing me to get OGSST's, OGS and my postdoc.

To Eric Hessels, thanks for all the letters and fun discussions. I can't look at a cake the same way as I used to!

To my parents to whom I can't thank you enough for the love and support all these years in everything from sports to academics. You both always ensured I was succeeding and supported my choices. To my mom for always respecting my decisions. You were always proud of my accomplishments and tried to make sure I would be secure and I thank you for that! Thank you mom for always being there to listen to what I was doing, whether it was intelligible or not and never being scarce with your loving words. To my dad for always respecting my judgment and being proud of my accomplishments. You never failed to let me know how proud of me you were, thank you.

To my brother I say thanks for everything. Thanks for the many years of discussion, friendship, love and support. 

To my grandmother, thank you for the love, support, food and wisdom. You were always proud of me and helped me understand how lucky I was for all that I had. You always had a kind word and the tastiest food! 

To my extended family I thank you for the years of love, support and encouragement. Whether it was picking me up at the train station from Ottawa, sending a card, making me food on a visit, throwing a party every time I visit or coming and visiting Bonnie and I in Toronto it always made me feel loved. 

To Igor Khavkine I'd like to say thank you for being a colleague as well as a mentor. Your knowledge and wisdom is always humbling and refreshing, but your enthusiasm and willingness to aid others with their work is exceptional. You were always willing to go though long discussions with me on any topic by email, phone or (in the best cases) over sushi and help in any way you could. I cannot thank you enough for your help, friendship and the many years of great badminton competitions.

To Devin Kovacz I'd like to say thank you for all the many years of friendship and intellectual sparring. I appreciated being able to call you up and have a stimulating discussion about my latest physics or non-physics idea and have you argue with me even if you agreed (in the rarest of cases). I would also like to thank you for the grammar help. Your money baby!

To Tzahi Yavin, thanks for sharing your knowledge and experiences making me a much wiser student. Thanks for always being willing to discuss any new idea I thought had merit regardless of whether it did.

To Matthew Guevremont, thanks for all the visits and the years of friendship. You've always been willing to give a helping hand even if it means driving a rickety van for 6 hours, thanks. 

To Joe Borely, thanks for friendship, encouragement and perseverance. You helped inspire me to stay a theorist, but thanks for helping me understand much more about experimental challenges.

To Luciano Lombardi, thanks for the many discussions, tea breaks and your friendship. Thanks for showing me some of the experimental side of physics and try really hard to question my beliefs. 

To Nav Sidhu, thanks for all the laughs, drinks and chess matches. Thanks for all the discussions and nights out, especially to all the concerts!

To Mauricio, Chris ,Sunny ,Alireza, Min, Carson, Scott, Laura, Brynle, Victoria, and Yan thanks for all the enjoyable discussions, encouragement and always being willing to hear my thoughts. Scott, enjoy both of the chairs with wheels, we can stop swapping them now.

To Carl Wolfe thanks for all the discussions about physics and parenting. Thanks for your friendship and willingness to hear me out on any new idea or rant that I had.

To my friends at CFI and FAC, Joe , Justin, Jenny, Brian, Ron, Emily and even Zak thanks for all the discussions, thought provoking discussions and the friendship. Your continued work makes me feel my thesis and research is more than a simple personal endeavor. Your doing great work, keep it up! A special thanks to Joe for the editing and grammar help! 

To my dog Emily, thanks for the long walks allowing me to clear my head and fill it with new perspectives and ideas. Thanks for listen to me practice my talks and always being ready to comfort me when things weren't going well.

I would like to thank the people at Sharcnet. There resources and helpful staff made this work possible.

Finally, I would like to thank the York Physics and Astronomy department staff for providing me with all the help and assistance I needed to navigate the bureaucracy. Special thanks to Marlene and Lauren for making everything simple enough that I could register or throw a movie night with pizza without any trouble.

==> abstract.tex <==
A fundamental prediction of the Dirac theory for electrons in strong electric fields is examined. When the electron's binding energy is sufficiently large the state becomes a pair creation resonance state, which is called a supercritical resonance. 

This resonance is similar in character to other resonances in atomic physics. It is parameterized by its energy and its lifetime. A numerical discretization technique, the mapped Fourier grid method (MFG) is extended to the Dirac equation and is used to solve for the resonance parameters of a quasimolecular supercritical 1S$\sigma$ state which arises, e.g., in a uranium-uranium collision. Direct methods using only the MFG method are shown to give reasonable estimates for the resonance parameters. Analytic continuation methods such as complex scaling (CS) of the coordinate or adding a complex absorbing potential (CAP) are then applied. They allow for more accurate determinations of the supercritical resonance parameters. 

The analytic continuation methods of smooth exterior scaling (SES) and CAP are then augmented by a Pad\'e approximant extrapolation. Both extrapolated methods are shown to give highly accurate results, with substantially smaller matrix sizes than direct analytic continuation calculations. They are also shown to give results in close agreement with each other. 

The (extrapolated) augmented analytic continuation methods are used to investigate the effects of higher-order couplings, beyond the monopole approximation. For the nearly charge symmetric system of U$^{92+}$-Cf$^{98+}$, it is shown that the S-D quadrupole coupling is the next dominant interaction after the monopole interaction.

Collisions near the Coulomb barrier, in which supercritical resonance states occur, are also calculated using the MFG. Results are presented for the collision of U$^{92+}$-U$^{92+}$ for a zero-impact-parameter Coulomb trajectory at a center-of-mass energy of 740MeV. The enhancement effects to the positron spectrum due to nuclear sticking at closest approach is examined. Results are given for sticking times of 2,5,10$\times10^{-21}$s. Nuclear sticking is shown to offer the possibility of demonstrating experimentally the existence of supercritical resonance states.


==> dedication.tex <==

\begin{flushright}
 \slshape \Large To Merissa, live your dreams
\end{flushright}
\normalfont
